Segmentation Rectification for Video Cutout via One-Class Structured Learning

Recent works on interactive video object cutout mainly focus on designing dynamic foreground-background (FB) classifiers for segmentation propagation. However, the research on optimally removing errors from the FB classification is sparse, and the errors often accumulate rapidly, causing significant errors in the propagated frames. In this work, we take the initial steps to addressing this problem, and we call this new task \emph{segmentation rectification}. Our key observation is that the possibly asymmetrically distributed false positive and false negative errors were handled equally in the conventional methods. We, alternatively, propose to optimally remove these two types of errors. To this effect, we propose a novel bilayer Markov Random Field (MRF) model for this new task. We also adopt the well-established structured learning framework to learn the optimal model from data. Additionally, we propose a novel one-class structured SVM (OSSVM) which greatly speeds up the structured learning process. Our method naturally extends to RGB-D videos as well. Comprehensive experiments on both RGB and RGB-D data demonstrate that our simple and effective method significantly outperforms the segmentation propagation methods adopted in the state-of-the-art video cutout systems, and the results also suggest the potential usefulness of our method in image cutout system.

==> abstract_CVPR.tex <==
\begin{abstract}
Recent works on interactive video object cutout mainly focus on designing dynamic foreground-background (FB) classifiers for segmentation propagation. In this paper,  we study the problem of removing the errors in these classifiers. The error of the FB classification can be uniquely decomposed into false positive (FP) and false negative (FN) errors. Different FB classifiers may have different biases toward either type of error. Common segmentation models consider the two types of errors equally, which might leave some errors unattended or incur new errors. To address this issue, we propose a novel {segmentation rectification} method to correct FB classification according to its intrinsic bias. Our method is based on a novel bilayer Markov random field (MRF) model that can handle FP and FN differently. The optimal model for a given classifier can be learned from the examples of FB classification using structured learning. In addition, we propose a novel one-class structured SVM (OSSVM) method which greatly speeds up the learning process. With our OSSVM method, we can learn our MRF model from thousands of training images in less than 0.1 second, in MATLAB on a normal PC. Comprehensive experiments demonstrate that our approach significantly outperforms state-of-the-art segmentation propagation methods used in previous systems. 
%Quantitative evaluation demonstrates that this approach, upon integration with existing classifiers used in previous systems, can lead 

%training of the classifiers relies on accurate motion estimation which often suffers from large displacement and topology changes. Consequently, the segmentation error could persist and tedious user interactions would be required to produce a satisfactory segmentation. 
%In this paper, we focus on reducing the errors from the foreground-background classification. In the previous video object cutout systems, Markov random field or matting has been applied to refine the classifier outputs. However, these models may not be fully compatible with the designed classifiers. 

%We propose \emph{data-driven segmentation rectification} to learn and integrate the classifier property into a segmentation model, and reduce the error from the underlying classifier effectively. Our novel approach is generic and can be applied to any classifier. 

\end{abstract}

==> discussion_CVPR.tex <==

\begin{figure}[!h]
	\centering
	\subfloat{\includegraphics[width=0.33\columnwidth]{imgs/failure_case/id9.jpg}
		\includegraphics[width=0.33\columnwidth]{imgs/failure_case/id9_edge_zoom1.png}
		\includegraphics[width=0.33\columnwidth]{imgs/failure_case/id9_trans.png}}\\\vspace{-2mm}
	\caption{Examples of failure cases I: spurious edges.}\label{FIG:SpuriousEdge}\vspace{-3mm}
	\centering
	\subfloat{\includegraphics[width=0.33\columnwidth]{imgs/failure_case/id364.png}
		\includegraphics[width=0.33\columnwidth]{imgs/failure_case/id365.png}
		\includegraphics[width=0.33\columnwidth]{imgs/failure_case/id365_all_trans.png}}\\\vspace{-3mm}
	\caption{Examples of failure cases II: abrupt emergence of object parts.}\label{FIG:SuddenParts}
\end{figure}
\section{Discussion}\label{SEC:DISC}

There are several vision tasks similar to the interactive video cutout~\cite{lee2011key,Papazoglou2013fastVseg,Jain2014supervoxelVseg}. In the context of computer vision, those problems can be classified as shape tracking problem, and errors are generally tolerable. They also require no user interactions. In contrast, the interactive video cutout problem does not tolerate errors in the segmentation. Thus, the current video cutout frameworks are particularly suitable for user interactions. In most of the works in vision~\cite{lee2011key,Papazoglou2013fastVseg,Jain2014supervoxelVseg}, global optimization frameworks are adopted. It has later been noted in~\cite{Bai09VideoSnapCut_SIGGRAPH} that the frame-by-frame optimization is more suitable for user to interact with the segmentation. Our method is proposed dedicatedly for video cutout. Its extension for generic video segmentation tasks has yet to be explored.


% Video segmentation
% VSB100 dataset

\section{Conclusion}\label{sec:conclusion}
We propose a novel generic approach to automatically rectify the propagated segmentation in video cutout systems. The core idea of our work is to incorporate a generic shape distance measure in a bilayer MRF framework learned from data to remove the intrinsic bias of the classifier in the segmentation propagation step. This work is motivated by our observation that different classifiers bias toward FP and FN differently, but they were treated equally in the previous video cutout systems. We found that FP and FN can be treated differently in our bilayer MRF, and the optimal form of the MRF can be learned from the data. Extensive evaluation demonstrates that our approach can significantly improve the state-of-the-art video cutout systems in segmentation accuracy.  

\iffalse
\section*{Appendix: A derivation to the one-class structured SVM}
We begin with the generic compact form of MRF. 
\iffalse
The unary term and the pairwise potential in an MRF can be written as:\vspace{-3mm}
\begin{equation}
\begin{split}
U_p(f_p) &= (\mathbf{w}_u\cdot\mathbf{x}_p) f_p,\\
V_{pq}(f_p,f_q) &= (\mathbf{w}_{pq}\cdot\mathbf{x}_{pq}) f_pf_q,
\end{split}
\end{equation}
where $\mathbf{x}_p$ can be viewed as the feature vector associated to a pixel $p$. $f_p$ is the pixel label and $\mathbf{w}_u$ is the weight vector for the features. Likewise, $\mathbf{x}_{pq}$ is the feature for a pair of pixels in the neighbourhood system. Accordingly, 
\fi
The MRF energy for one image can be written as a inner product form w.r.t. the weights $\{\mathbf{w}_u,~\mathbf{w}_{pq}\}$:
\begin{equation}
%\begin{split}
E(f|\mathbf{w},\mathbf{x}) %&= \sum_p \mathbf{w}_u \cdot (\mathbf{x}_p f_p) + \sum_{\{p,q\}\in \mathcal{N}} \mathbf{w}_{pq}\cdot (\mathbf{x}_{pq} f_pf_q)\\
                = \mathbf{w}\cdot \mathbf{\Psi}(\mathbf{x},\mathbf{f})
%\end{split}
\end{equation}
where $\mathbf{w} = [\mathbf{w}_u,\mathbf{w}_{pq}]$ and $\mathbf{\Psi}(\mathbf{x},\mathbf{f}) = [\sum_p \mathbf{x}_p f_p,\sum_{\{p,q\}\in \mathcal{N}} \mathbf{x}_{pq} f_pf_q]^T$, $\mathbf{x}_p$ and $\mathbf{x}_{pq}$ are the features for unary and pairwise potential.

We expect the MRF energy to be as small as possible for the ground truth $\mathbf{f}^*$ and we expect it to be as large as possible for other $\mathbf{f}$. This principle can be used for learning the weight vector $\mathbf{w}$ from data, and it can be expressed as:\vspace{-3mm}
\begin{equation}\label{EQ:2C_SSVM}
\begin{split}
\min_{\mathbf{w},b,\vec{\xi}}~& {1\over2}\|\mathbf{w}\|^2 + {C\over N}\sum_{k=1}^N \xi_k \\
\hbox{s.t.:}~&  \begin{array}{r}
                   2\mathbf{w}\cdot\mathbf{\Psi}(\mathbf{x}_k,\mathbf{f}_k)-b\geq +1 - \xi_k %, & \hbox{if~} \mathbf{f}_k \hbox{~is bad} 
                   \\
                   2\mathbf{w}\cdot\mathbf{\Psi}(\mathbf{x}_k,\mathbf{f}_k^*)-b\leq -1 + \xi_k, % & \hbox{if~} \mathbf{f}_k \hbox{~is good}
\end{array}
\end{split}
\end{equation}
where the constants $b$ is a bias in conventional decision function and $\xi_k$ is a lack variable that tolerates errors in the training data. In the above model, the margin that separates the positive and negative samples are  maximized by minimizing $\|\mathbf{w}\|^2$ \cite{Taskar05LargeMargin,Tsochantaridis05LargeMarginSSVM}. 

Knowing that the samples are paired, we therefore can combine the constraints for each pair of samples to yield the following constraint: %\vspace{-3mm}
\begin{equation}\label{EQ:SSVM_Constr}
                   \mathbf{w}\cdot\mathbf{\Psi}(\mathbf{x}_k,\mathbf{f}_k)-\mathbf{w}\cdot\mathbf{\Psi}(\mathbf{x}_k,\mathbf{f}^*_k)\geq 1 - \xi_k
\end{equation}
With the additional requirements of positiveness and boundedness of $\mathbf{w}$, we can obtain the conventional SSVM \cite{Tsochantaridis05LargeMarginSSVM,Taskar05LargeMargin,Szummer08LearnCRFbyGC,Joachims2009CuttingPlaneSSVM}.
\iffalse
\vspace{-5mm}
\begin{equation}\label{EQ:SSVM}
\begin{split}
\min_{\mathbf{w},\vec{\xi}}~& {1\over2}\|\mathbf{w}\|^2 + {C\over N}\sum_{k=1}^N \xi_k \\
\hbox{s.t.:}~&  \forall k,~\mathbf{w}\cdot\mathbf{\Psi}(\mathbf{x}_k,\mathbf{f}_k)-\mathbf{w}\cdot\mathbf{\Psi}(\mathbf{x}_k,\mathbf{f}^*_k)\geq 1 - \xi_k\\
            ~&  \sum_i w_i=1, \mathbf{w}\geq0, \forall k,~\xi_k\geq0
\end{split}
\end{equation}
In the above model, positiveness and boundedness of $\mathbf{w}$ are further considered.


We can insert the notations of the structured learning used in Eqs. (\ref{EQ:2C_SVM}) into the one-class SVM~\cite{Scholkopf01oneclassSVM} to immediately obtain a structured learning formulation in the form of conventional two-class SVM~\cite{Scholkopf01oneclassSVM}.
\fi

In the following, we show how $\mathbf{\Phi}$ can be obtained and how the main constraint (second line) above can be derived according to the basic requirement of structured learning.
\iffalse

In the structured learning, we require $\mathbf{w}\cdot\mathbf{\Psi}(\mathbf{x}_k,\mathbf{f}^*_k)$ to be as small as possible for good $\mathbf{f}^*_k$, i.e.:\vspace{-2mm}
\begin{equation}\label{eq:SSVM_constraint}
\mathbf{w}\cdot\mathbf{\Psi}(\mathbf{x}_k,\mathbf{f}^*_k)-b\leq -1+\xi_k
\end{equation}
\fi

Let us consider a transformation:
$\mathbf{\Phi}(\mathbf{x}_k,\mathbf{f}^*_k)=M-\mathbf{\Psi}(\mathbf{x}_k,\mathbf{f}^*_k)$, where $M$ is a sufficiently large positive constant to ensure $\mathbf{\Phi}(\mathbf{x}_k,\mathbf{f}^*_k)\geq 0$. Substituting the $\mathbf{\Phi}$ into the constraint in Eq. (\ref{EQ:2C_SSVM}), we have:\vspace{-1mm}
\begin{equation}
\begin{split}
&M(\mathbf{1}^T\mathbf{w})-\mathbf{w}\cdot\mathbf{\Phi}(\mathbf{x}_k,\mathbf{f}^*_k)-b\leq -1+\xi_k\\
&\Leftrightarrow \mathbf{w}\cdot\mathbf{\Phi}(\mathbf{x}_k,\mathbf{f}^*_k)\geq 1+M-b-\xi_k
\end{split}
\end{equation}
where we have applied the constraint $\sum_i w_i = 1$. 

Let $\beta = M-b$, $\hat{\xi}_k = \xi_k-1$ we obtain an alternative form of structured learning as follows
\begin{equation}\label{EQ:OSSVM_np}
\begin{split}
\min_{\mathbf{w},\beta,\vec{\hat{\xi}}}~& {1\over2}\|\mathbf{w}\|^2 + {C\over N}\sum_{k=1}^N (\hat{\xi}_k-\beta)  \\
\hbox{s.t.:}~&  \forall k,~ \mathbf{w}\cdot\mathbf{\Phi}(\mathbf{x}_k,f^*_k)\geq \beta-\hat{\xi}_k, \\
              &  \sum_i w_i=1, \mathbf{w}\geq 0, \forall k,~\beta-\hat{{\xi}}_k\geq 0 \\
\end{split}
\end{equation}
Please note that the above form follows the the one-class SVM~\cite{Scholkopf01oneclassSVM} exactly. Additionally, note that the good samples are considered as positive samples in this model, and $\mathbf{\Phi}$ is not the MRF potential we used previously. 

Since we are not interested in the value of $\beta$, we may combine the slack variables to be $\varepsilon_k = \beta-\hat{\xi}_k$, which has to be still nonnegative for a sufficiently large $M$. 

\fi
%Additionally, we require the weight for the edge cue to be as large as possible, since the edge cue is almost always valid. This prior can be easily incorporated in the above quadratic programming as a linear term to arrive at:
%\begin{equation}\label{EQ:OSSVM_wp}
%\begin{split}
%\min_{\mathbf{w},\beta,\vec{\hat{\xi}}}~& {1\over2}\|\mathbf{w}\|^2 + {C\over N}\sum_{k=1}^N (\hat{\xi}_k-\beta)-w^{edge}  \\
%\hbox{s.t.:}~&  \forall k,~ \mathbf{w}\cdot\mathbf{\Phi}(\mathbf{x}_k,f^*_k)\geq \beta-\hat{\xi}_k \\
%             &  \forall k,~\beta-{\xi}_k\geq 0 \\
%             &  \sum_i w_i=1, \mathbf{w}\geq 0
%\end{split}
%\end{equation}
%where the last term in the objective function is our prior. An experimental validation of this prior is presented in the experiment section.



